Inferring Algebraic Effects

We present a complete polymorphic effect inference algorithm for an ML-style language with handlers of not only exceptions, but of any other algebraic effect such as input & output, mutable references and many others. Our main aim is to offer the programmer a useful insight into the effectful behaviour of programs. Handlers help here by cutting down possible effects and the resulting lengthy output that often plagues precise effect systems. Additionally, we present a set of methods that further simplify the displayed types, some even by deliberately hiding inferred information from the programmer.

==> macros.tex <==
\makeatletter
\providecommand*{\cupdot}{%
  \mathbin{%
    \mathpalette\@cupdot{}%
  }%
}
\newcommand*{\@cupdot}[2]{%
  \ooalign{%
    $\m@th#1\cup$\cr
    \sbox0{$#1\cup$}%
    \dimen@=\ht0 %
    \sbox0{$\m@th#1\cdot$}%
    \advance\dimen@ by -\ht0 %
    \dimen@=.5\dimen@
    \hidewidth\raise\dimen@\box0\hidewidth
  }%
}

\DeclareFontFamily{U}{mathb}{\hyphenchar\font45}
\DeclareFontShape{U}{mathb}{m}{n}{
      <5> <6> <7> <8> <9> <10> gen * mathb
      <10.95> mathb10 <12> <14.4> <17.28> <20.74> <24.88> mathb12
      }{}
\DeclareSymbolFont{mathb}{U}{mathb}{m}{n}
\DeclareMathSymbol{\dotminus}{2}{mathb}{"01}

\providecommand*{\bigcupdot}{%
  \mathop{%
    \vphantom{\bigcup}%
    \mathpalette\@bigcupdot{}%
  }%
}
\newcommand*{\@bigcupdot}[2]{%
  \ooalign{%
    $\m@th#1\bigcup$\cr
    \sbox0{$#1\bigcup$}%
    \dimen@=\ht0 %
    \advance\dimen@ by -\dp0 %
    \sbox0{\scalebox{2}{$\m@th#1\cdot$}}%
    \advance\dimen@ by -\ht0 %
    \dimen@=.5\dimen@
    \hidewidth\raise\dimen@\box0\hidewidth
  }%
}
\makeatother


% Meta-syntax
\newcommand{\bnfis}{\mathrel{\;{:}{:}\!=}\;}
\newcommand{\bnfor}{\mathrel{\;\big|\;}}
\newcommand{\defeq}{\mathrel{\;\stackrel{\text{def}}{=}\;}}
\newcommand{\fra}[1]{\forall #1 .\ }
\newcommand{\exs}[1]{\exists #1 .\ }
\newcommand{\rulename}[1]{{\mdseries \small \textsc{#1}}}
\newcommand{\set}[1]{\{ #1 \}}
\newcommand{\step}{\leadsto}

% Types
\newcommand{\type}[1]{\mathtt{#1}}
\newcommand{\boolty}{\type{bool}}
\newcommand{\natty}{\type{nat}}
\newcommand{\unitty}{\type{unit}}
\newcommand{\emptyty}{\type{empty}}
\newcommand{\listty}{\;\type{list}}
\newcommand{\stringty}{\type{string}}
\renewcommand{\to}[1][]{
  \def\arg{#1}%
  \ifx\arg\emptyarg\rightarrow\else\xrightarrow{#1}\fi%
}
\newcommand{\hto}[1][]{
  \def\arg{#1}%
  \ifx\arg\emptyarg\Rightarrow\else\xRightarrow{#1}\fi%
}
\newcommand{\C}{\underline{C}}
\newcommand{\D}{\underline{D}}
\newcommand{\Drt}{\Delta}
\newcommand{\drt}{\delta}
\newcommand{\Rgn}{R}
\newcommand{\wild}{\top}
\makeatletter
\newcommand{\rgn}{\@ifstar{\dot{\rho}}{\rho}}
\makeatother
\newcommand{\prs}{\psi}
\newcommand{\uniq}[2]{\bigcupdot\nolimits_{#1} #2}
\newcommand{\varuniq}[2]{\bigcupdot_{#1} #2}

% Expressions and computations
\newcommand{\kord}[1]{\mathtt{#1}}
\newcommand{\kop}[1]{\;\mathtt{#1}\;}
\newcommand{\kpre}[1]{\mathtt{#1}\;}
\newcommand{\kpost}[1]{\;\mathtt{#1}}

\newcommand{\absurd}{\kpre{absurd}}
\newcommand{\case}{\mathop{\text{\texttt{|}}}}
\newcommand{\cont}[2]{(#1.\,#2)}
\newcommand{\fls}{\kord{false}}
\newcommand{\fun}[1]{\kpre{fun} #1 \mapsto}
\newcommand{\handler}{\kpre{handler}}
\newcommand{\hash}[2]{#1\text{\texttt{\char35}}#2}
\newcommand{\iszero}{\kpre{iszero}}
\newcommand{\letin}[1]{\kpre{let} #1 \kop{in}}
\newcommand{\letrecin}[1]{\kpre{let} \kpre{rec} #1 \kop{in}}
\newcommand{\letvalin}[1]{\kpre{let} \kpre{val} #1 \kop{in}}
\newcommand{\call}[4]{{\hash{#1}{#2}\,{#3}\, #4}}
\newcommand{\op}{\mathtt{op}}
\newcommand{\inst}{\mathtt{ins}}
\newcommand{\pred}{\kpre{pred}}
\newcommand{\tru}{\kord{true}}
\newcommand{\unt}{\kord{\text{\texttt{()}}}}
\newcommand{\val}{\kpre{val}}
\newcommand{\withhandle}[2]{\kpre{with} #1 \kop{handle} #2}
\renewcommand{\ifthenelse}[3]{\kpre{if} #1 \kop{then} #2 \kop{else} #3}
\renewcommand{\succ}{\kpre{succ}}

% Judgements
\newcommand{\goesto}{\leadsto}
\newcommand{\ctx}{\Gamma}
\newcommand{\pctx}{\Xi}
\newcommand{\ent}[1][]{\vdash_{#1}}
\newcommand{\T}{\mathrel{:}}
\newcommand{\E}{\mathrel{!}}
\newcommand{\while}{\mid}
\renewcommand{\le}{\leqslant}

% Special sets
\newcommand{\cstr}{\mathcal{C}}
\newcommand{\queue}{\mathcal{Q}}
\newcommand{\prms}{\Psi}
\newcommand{\ops}{\mathcal{O}}
\newcommand{\insts}{\mathcal{I}}
\newcommand{\types}[2][A]{\llbracket #1 \mid #2 \rrbracket}
\newcommand{\sol}{\sigma}
\newcommand{\sig}{\Sigma}
\newcommand{\extend}[2]{#1 \cup \set{#2}}

% Names
\newcommand{\Eff}{\emph{Eff}\xspace}
\newcommand{\unify}{\kord{unify}}
\newcommand{\pos}{\kord{pos}}
\renewcommand{\neg}{\kord{neg}}
\newcommand{\gc}[1][P, N]{\kord{gc}_{#1}}

